SIDOD: A Synthetic Image Dataset for 3D Object Pose Recognition with Distractors

We present a new, publicly-available image dataset generated by the NVIDIA Deep Learning Data Synthesizer intended for use in object detection, pose estimation, and tracking applications. This dataset contains 144k stereo image pairs that synthetically combine 18 camera viewpoints of three photorealistic virtual environments with up to 10 objects (chosen randomly from the 21 object models of the YCB dataset [1]) and flying distractors. Object and camera pose, scene lighting, and quantity of objects and distractors were randomized. Each provided view includes RGB, depth, segmentation, and surface normal images, all pixel level. We describe our approach for domain randomization and provide insight into the decisions that produced the dataset.

==> data/001980-left-json.tex <==
{
	"camera_data":
	{
		"location_worldframe": [ -262.2506103515625, 769.69580078125, 197.47160339355469 ],
		"quaternion_xyzw_worldframe": [ 0.25139999389648438, 0.091600000858306885, -0.90530002117156982, 0.32980000972747803 ]
	},
	"objects": [
		{
			"class": "003_cracker_box_16k",
			"visibility": 0.98919999599456787,
			"location": [ 23.760599136352539, 9.8744001388549805, 64.910797119140625 ],
			"quaternion_xyzw": [ 0.050999999046325684, 0.99400001764297485, -0.06210000067949295, 0.073899999260902405 ],
			"pose_transform": [
				[ 0.14059999585151672, -0.13099999725818634, -0.9814000129699707, 0 ],
				[ -0.98390001058578491, 0.092200003564357758, -0.15320000052452087, 0 ],
				[ -0.11050000041723251, -0.98710000514984131, 0.11590000241994858, 0 ],
				[ 23.760599136352539, 9.8744001388549805, 64.910896301269531, 1 ]
			],
			"cuboid_centroid": [ 23.760700225830078, 9.8744001388549805, 64.910896301269531 ],
			"projected_cuboid_centroid": [ 761.18408203125, 386.85400390625 ],
			"bounding_box":
			{
				"top_left": [ 251.43569946289063, 639.42718505859375 ],
				"bottom_right": [ 535.18670654296875, 889.8201904296875 ]
			},
			"cuboid": [
				[ 15.01609992980957, -0.37380000948905945, 61.368000030517578 ],
				[ 31.155300140380859, -1.8860000371932983, 63.881301879882813 ],
				[ 33.514499664306641, 19.182199478149414, 61.407398223876953 ],
				[ 17.375200271606445, 20.694299697875977, 58.894199371337891 ],
				[ 14.006899833679199, 0.56660002470016479, 68.414299011230469 ],
				[ 30.146099090576172, -0.94559997320175171, 70.927597045898438 ],
				[ 32.505298614501953, 20.122600555419922, 68.453697204589844 ],
				[ 16.366100311279297, 21.634700775146484, 65.940399169921875 ]
			],
			"projected_cuboid": [
				[ 667.95867919921875, 265.32080078125 ],
				[ 854.63482666015625, 247.32170104980469 ],
				[ 899.2393798828125, 509.9547119140625 ],
				[ 706.62420654296875, 539.91748046875 ],
				[ 637.268310546875, 276.36111450195313 ],
				[ 806.48748779296875, 259.75900268554688 ],
				[ 844.76080322265625, 495.80780029296875 ],
				[ 670.651611328125, 522.02947998046875 ]
			]
		},
		{
			"class": "008_pudding_box_16k",
			"visibility": 0.88370001316070557,
			"location": [ -2.4015998840332031, 12.185500144958496, 64.190696716308594 ],
			"quaternion_xyzw": [ 0.14910000562667847, 0.76620000600814819, 0.22920000553131104, 0.58160001039505005 ],
			"pose_transform": [
				[ 0.9595000147819519, 0.17779999971389771, -0.21850000321865082, 0 ],
				[ -0.27910000085830688, 0.4950999915599823, -0.82279998064041138, 0 ],
				[ 0.038199998438358307, -0.85049998760223389, -0.52460002899169922, 0 ],
				[ -2.4015998840332031, 12.185500144958496, 64.190696716308594, 1 ]
			],
			"cuboid_centroid": [ -2.4015998840332031, 12.185600280761719, 64.190597534179688 ],
			"projected_cuboid_centroid": [ 451.25839233398438, 415.822998046875 ],
			"bounding_box":
			{
				"top_left": [ 328.86248779296875, 405.95950317382813 ],
				"bottom_right": [ 507.6416015625, 495.22430419921875 ]
			},
			"cuboid": [
				[ -1.9707000255584717, 11.521599769592285, 56.738498687744141 ],
				[ 1.2015999555587769, 5.8951001167297363, 66.090103149414063 ],
				[ 0.85879999399185181, 13.533699989318848, 70.802299499511719 ],
				[ -2.313499927520752, 19.160200119018555, 61.450698852539063 ],
				[ -5.6620001792907715, 10.837400436401367, 57.5791015625 ],
				[ -2.4897000789642334, 5.210899829864502, 66.930702209472656 ],
				[ -2.8324999809265137, 12.849499702453613, 71.642898559570313 ],
				[ -6.0047998428344727, 18.47599983215332, 62.29119873046875 ]
			],
			"projected_cuboid": [
				[ 453.31719970703125, 425.98611450195313 ],
				[ 493.96438598632813, 338.5181884765625 ],
				[ 489.31600952148438, 416.83248901367188 ],
				[ 451.07818603515625, 509.510986328125 ],
				[ 404.45980834960938, 414.58099365234375 ],
				[ 451.42388916015625, 329.80499267578125 ],
				[ 449.62799072265625, 407.7738037109375 ],
				[ 405.94790649414063, 497.84228515625 ]
			]
		},
		{
			"class": "005_tomato_soup_can_16k",
			"visibility": 1,
			"location": [ -24.881500244140625, 3.9302000999450684, 73.557899475097656 ],
			"quaternion_xyzw": [ -0.27469998598098755, 0.34000000357627869, 0.40389999747276306, 0.803600013256073 ],
			"pose_transform": [
				[ 0.3246999979019165, 0.71609997749328613, 0.61790001392364502, 0 ],
				[ 0.44249999523162842, 0.46230000257492065, -0.76840001344680786, 0 ],
				[ 0.83590000867843628, -0.52289998531341553, 0.16680000722408295, 0 ],
				[ -24.881500244140625, 3.9302000999450684, 73.557899475097656, 1 ]
			],
			"cuboid_centroid": [ -24.881500244140625, 3.9302000999450684, 73.557899475097656 ],
			"projected_cuboid_centroid": [ 220.16259765625, 311.04269409179688 ],
			"bounding_box":
			{
				"top_left": [ 249.27070617675781, 149.59550476074219 ],
				"bottom_right": [ 371.82611083984375, 288.8114013671875 ]
			},
			"cuboid": [
				[ -18.028099060058594, 5.2557997703552246, 73.900001525878906 ],
				[ -21.022300720214844, 2.1278998851776123, 79.098899841308594 ],
				[ -29.536500930786133, 7.4538998603820801, 77.39959716796875 ],
				[ -26.542200088500977, 10.58180046081543, 72.200798034667969 ],
				[ -20.226400375366211, 0.40659999847412109, 69.716300964355469 ],
				[ -23.220800399780273, -2.7214000225067139, 74.91510009765625 ],
				[ -31.734899520874023, 2.6045999526977539, 73.215896606445313 ],
				[ -28.740699768066406, 5.732600212097168, 68.016998291015625 ]
			],
			"projected_cuboid": [
				[ 292.60391235351563, 324.63180541992188 ],
				[ 275.84201049804688, 290.664306640625 ],
				[ 186.86030578613281, 343.97650146484375 ],
				[ 197.60960388183594, 382.5823974609375 ],
				[ 257.13510131835938, 274.4796142578125 ],
				[ 241.89849853515625, 242.09530639648438 ],
				[ 147.04440307617188, 297.32659912109375 ],
				[ 155.41059875488281, 334.74160766601563 ]
			]
		},
		{
			"class": "024_bowl_16k",
			"visibility": 0.98360002040863037,
			"location": [ -11.874500274658203, -11.65839958190918, 88.011299133300781 ],
			"quaternion_xyzw": [ -0.14980000257492065, 0.90380001068115234, 0.12690000236034393, -0.38029998540878296 ],
			"pose_transform": [
				[ -0.72539997100830078, 0.11559999734163284, -0.678600013256073, 0 ],
				[ -0.66589999198913574, -0.36719998717308044, 0.6492999792098999, 0 ],
				[ 0.17419999837875366, -0.92290002107620239, -0.34340000152587891, 0 ],
				[ -11.874500274658203, -11.65839958190918, 88.011299133300781, 1 ]
			],
			"cuboid_centroid": [ -11.874500274658203, -11.65839958190918, 88.011299133300781 ],
			"projected_cuboid_centroid": [ 376.35760498046875, 168.24560546875 ],
			"bounding_box":
			{
				"top_left": [ 128.214599609375, 307.65719604492188 ],
				"bottom_right": [ 203.472900390625, 449.6044921875 ]
			},
			"cuboid": [
				[ -22.618000030517578, -16.223100662231445, 86.821197509765625 ],
				[ -11.88539981842041, -10.304400444030762, 76.356101989746094 ],
				[ -12.843299865722656, -5.2274999618530273, 78.244903564453125 ],
				[ -23.576000213623047, -11.146200180053711, 88.70989990234375 ],
				[ -10.905799865722656, -18.089199066162109, 97.777603149414063 ],
				[ -0.17299999296665192, -12.170599937438965, 87.312599182128906 ],
				[ -1.1310000419616699, -7.0936999320983887, 89.201400756835938 ],
				[ -11.863800048828125, -13.012399673461914, 99.666397094726563 ]
			],
			"projected_cuboid": [
				[ 279.88308715820313, 126.46420288085938 ],
				[ 360.42840576171875, 166.33489990234375 ],
				[ 353.91079711914063, 218.67909240722656 ],
				[ 275.8485107421875, 173.48210144042969 ],
				[ 394.32080078125, 127.88700103759766 ],
				[ 478.47671508789063, 162.92509460449219 ],
				[ 470.25930786132813, 208.91209411621094 ],
				[ 388.56109619140625, 169.70939636230469 ]
			]
		},
		{
			"class": "005_tomato_soup_can_16k",
			"visibility": 0.96719998121261597,
			"location": [ 0.35609999299049377, -8.7483997344970703, 96.996101379394531 ],
			"quaternion_xyzw": [ 0.0088999997824430466, -0.66820001602172852, -0.39219999313354492, 0.63220000267028809 ],
			"pose_transform": [
				[ -0.85180002450942993, 0.51289999485015869, 0.10689999908208847, 0 ],
				[ -0.20059999823570251, -0.50770002603530884, 0.83789998292922974, 0 ],
				[ -0.48399999737739563, -0.69220000505447388, -0.53530001640319824, 0 ],
				[ 0.35609999299049377, -8.7483997344970703, 96.996101379394531, 1 ]
			],
			"cuboid_centroid": [ 0.35609999299049377, -8.7482995986938477, 96.996002197265625 ],
			"projected_cuboid_centroid": [ 482.81930541992188, 200.71760559082031 ],
			"bounding_box":
			{
				"top_left": [ 149.78289794921875, 436.63681030273438 ],
				"bottom_right": [ 249.70370483398438, 526.71929931640625 ]
			},
			"cuboid": [
				[ -5.6711001396179199, -12.25469970703125, 97.466102600097656 ],
				[ -4.314000129699707, -8.8198003768920898, 91.797203063964844 ],
				[ 0.61559998989105225, -1.7690000534057617, 97.249603271484375 ],
				[ -0.74150002002716064, -5.2038998603820801, 102.91850280761719 ],
				[ 0.0966000035405159, -15.727700233459473, 96.742500305175781 ],
				[ 1.4536999464035034, -12.292799949645996, 91.073600769042969 ],
				[ 6.3833999633789063, -5.2420001029968262, 96.5260009765625 ],
				[ 5.0261998176574707, -8.6768999099731445, 102.19490051269531 ]
			],
			"projected_cuboid": [
				[ 435.30239868164063, 173.41659545898438 ],
				[ 443.89859008789063, 196.19590759277344 ],
				[ 484.8616943359375, 256.02731323242188 ],
				[ 474.46450805664063, 231.1593017578125 ],
				[ 480.76559448242188, 145.1177978515625 ],
				[ 492.260009765625, 166.31640625 ],
				[ 530.79779052734375, 228.28399658203125 ],
				[ 517.77880859375, 204.77879333496094 ]
			]
		},
		{
			"class": "008_pudding_box_16k",
			"visibility": 0.11490000039339066,
			"location": [ 18.281400680541992, -12.156200408935547, 102.84709930419922 ],
			"quaternion_xyzw": [ -0.22709999978542328, 0.91310000419616699, -0.086900003254413605, -0.32739999890327454 ],
			"pose_transform": [
				[ -0.55830001831054688, -0.30739998817443848, -0.77060002088546753, 0 ],
				[ -0.68250000476837158, -0.35780000686645508, 0.63730001449584961, 0 ],
				[ 0.47170001268386841, -0.88169997930526733, 0.0099999997764825821, 0 ],
				[ 18.281400680541992, -12.156200408935547, 102.84709930419922, 1 ]
			],
			"cuboid_centroid": [ 18.281400680541992, -12.156200408935547, 102.84709930419922 ],
			"projected_cuboid_centroid": [ 616.5418701171875, 179.20599365234375 ],
			"bounding_box":
			{
				"top_left": [ 133.43119812011719, 563.2034912109375 ],
				"bottom_right": [ 226.17469787597656, 673.4813232421875 ]
			},
			"cuboid": [
				[ 15.446999549865723, -18.740699768066406, 105.03130340576172 ],
				[ 23.204099655151367, -14.673600196838379, 97.788398742675781 ],
				[ 18.967899322509766, -6.7543001174926758, 97.698402404785156 ],
				[ 11.210800170898438, -10.821399688720703, 104.94139862060547 ],
				[ 17.594999313354492, -17.558099746704102, 107.99579620361328 ],
				[ 25.352100372314453, -13.491000175476074, 100.75279998779297 ],
				[ 21.115800857543945, -5.5715999603271484, 100.66290283203125 ],
				[ 13.358799934387207, -9.6386995315551758, 107.90579986572266 ]
			],
			"projected_cuboid": [
				[ 592.9730224609375, 132.93699645996094 ],
				[ 662.27471923828125, 154.73350524902344 ],
				[ 629.13531494140625, 216.89419555664063 ],
				[ 562.0615234375, 190.7886962890625 ],
				[ 605.14971923828125, 145.11149597167969 ],
				[ 673.2882080078125, 167.14190673828125 ],
				[ 641.13409423828125, 227.48300170898438 ],
				[ 575.09759521484375, 201.38429260253906 ]
			]
		},
		{
			"class": "036_wood_block_16k",
			"visibility": 0.60000002384185791,
			"location": [ 19.865200042724609, -3.6085000038146973, 86.125 ],
			"quaternion_xyzw": [ 0.38890001177787781, 0.47699999809265137, 0.045899998396635056, 0.78689998388290405 ],
			"pose_transform": [
				[ 0.78630000352859497, -0.56819999217987061, 0.24259999394416809, 0 ],
				[ 0.54079997539520264, 0.44319999217987061, -0.71490001678466797, 0 ],
				[ -0.2987000048160553, -0.69330000877380371, -0.6557999849319458, 0 ],
				[ 19.865200042724609, -3.6085000038146973, 86.125, 1 ]
			],
			"cuboid_centroid": [ 19.865200042724609, -3.6085000038146973, 86.125 ],
			"projected_cuboid_centroid": [ 657.1793212890625, 237.814697265625 ],
			"bounding_box":
			{
				"top_left": [ 129.23829650878906, 580.26422119140625 ],
				"bottom_right": [ 339.12298583984375, 722.22869873046875 ]
			},
			"cuboid": [
				[ 22.781999588012695, -11.344499588012695, 77.262199401855469 ],
				[ 17.93120002746582, -15.319899559020996, 83.674598693847656 ],
				[ 24.086700439453125, -1.0306999683380127, 97.19000244140625 ],
				[ 28.937599182128906, 2.9447999000549316, 90.777702331542969 ],
				[ 15.643699645996094, -6.1863999366760254, 75.05999755859375 ],
				[ 10.792799949645996, -10.161899566650391, 81.472396850585938 ],
				[ 16.948400497436523, 4.1273999214172363, 94.987800598144531 ],
				[ 21.799299240112305, 8.1028003692626953, 88.575401306152344 ]
			],
			"projected_cuboid": [
				[ 706.503173828125, 157.21029663085938 ],
				[ 644.61309814453125, 129.35800170898438 ],
				[ 670.373291015625, 261.85400390625 ],
				[ 724.86920166015625, 294.91879272460938 ],
				[ 640.09539794921875, 206.68829345703125 ],
				[ 581.75830078125, 174.18879699707031 ],
				[ 617.0596923828125, 303.3778076171875 ],
				[ 669.0504150390625, 340.27090454101563 ]
			]
		}
	]
}

==> table1.tex <==
\renewcommand{\rb}[1]{\rotatebox{0}{#1}}%
\begin{table*}[ht]
    % \centering
    \begin{tabular}{rrrc|ccccccccc}
    % Dataset & \multicolumn{1}{p{0.1cm}}{\centering \# \\objects}  &  \multicolumn{1}{p{0.1cm}}{\centering \# \\frames} & Description & 
%     \rb{depth} & \rb{stereo} & \rb{\multicolumn{1}{p{0.5cm}}{\centering 3D \\ pose}}  &
%   \rb{\multicolumn{1}{p{0.5cm}}{\centering full \\ rotation}}  & \rb{occlusion} & \rb{\multicolumn{1}{p{0.5cm}}{\centering extreme \\ lighting}}  & 
%     \rb{\multicolumn{1}{p{0.5cm}}{\centering segment \\ ation}}  & \rb{\multicolumn{1}{p{0.5cm}}{\centering bbox \\ coords}} & \rb{\multicolumn{1}{p{0.5cm}}{\centering flying \\ distractors}} \\
    Dataset & \# objects & \# frames & Description & 
    \rb{dep.} & \rb{ster.} & \rb{pose} &
    \rb{rot.} & \rb{occ.} & \rb{e.l.} & 
    \rb{seg.} & \rb{coor.} & \rb{f.d.}\\
    \hline
    
    UW RGB~\cite{lai2011large} & 300 & 250k & various & 
    \cmark & \xmark & \cmark & \cmark & \xmark & \xmark & \xmark & \xmark & \xmark \\
    
    LINEMOD~\cite{hinterstoisser2012model} & 15 & 18k & various & 
    \cmark & \xmark & \cmark & \cmark & \xmark & \xmark & \xmark & \xmark & \xmark \\
    
    Pascal3D+~\cite{xiang2014beyond} & 12 & 30k & various & 
    \xmark & \xmark & \cmark & \xmark & \cmark & \cmark & \xmark & \xmark & \xmark \\
    
   % Brachman et al.~\cite{brachmann2014learning} & 20 & 10k & various & 
  %  \cmark & \xmark & \cmark & \cmark & \cmark & \cmark & \xmark & \xmark & \xmark \\
    
    Rutgers APC~\cite{rennie2016dataset} & 24 & 10k & warehouse & 
    \cmark & \xmark & \cmark & \xmark & \xmark & \xmark & \xmark & \xmark & \xmark \\
    
    T-LESS~\cite{hodan2017t} & 30 & 10k & industrial & 
    \cmark & \xmark & \cmark & \cmark & \cmark & \xmark & \xmark & \xmark & \xmark \\
    
    YCB Video~\cite{xiang2017posecnn} & 21 & 134k & household & 
    \cmark & \xmark & \cmark & \cmark & \cmark & \xmark & \cmark & \cmark & \xmark \\
    
    Falling Things~\cite{tremblay2018falling} & 21 & 60k & household & 
    \cmark & \cmark & \cmark & \cmark & \cmark & \cmark & \cmark & \cmark & \xmark \\
    
    SIDOD & 21 & 144k & household & 
    \cmark & \cmark & \cmark & \cmark & \cmark & \cmark & \cmark & \cmark & \cmark \\
         & 
    \end{tabular}
    \caption{Object pose and detection datasets with at least 10,000 frames. Column labels represent depth image (dep.), stereo images (ster.), 3D pose (pose), full rotation (rot.), occlusion (occ.), extreme lighting (e.l.), segmentation (seg.), bounding box coodinates (coor.), and flying distractors (f.d.).} %TODO: finish caption.}
    \label{tab:comparison}
\end{table*}
